CHESS: Contextual Harnessing for Efficient SQL Synthesis

Translating natural language questions into SQL queries, known as text-to-SQL, is a long-standing research problem. Effective text-to-SQL synthesis can become very challenging due to (i) the extensive size of database catalogs (descriptions of tables and their columns) and database values, (ii) reasoning over large database schemas, (iii) ensuring the functional validity of the generated queries, and (iv) navigating the ambiguities of natural language questions. We introduce CHESS, a Large Language Model (LLM) based multi-agent framework for efficient and scalable SQL synthesis, comprising four specialized agents, each targeting one of the aforementioned challenges: the Information Retriever (IR) extracts relevant data, the Schema Selector (SS) prunes large schemas, the Candidate Generator (CG) generates high-quality candidates and refines queries iteratively, and the Unit Tester (UT) validates queries through LLM-based natural language unit tests. Our framework offers configurable features that adapt to various deployment constraints, including 1) Supporting industrial-scale databases: leveraging the Schema Selector agent, CHESS efficiently narrows down very large database schemas into manageable sub-schemas, boosting system accuracy by approximately $2\%$ and reducing the number of LLM tokens by $\times 5$. 2) State-of-the-Art privacy-preserving performance: Among the methods using open-source models, CHESS achieves state-of-the-art performance, resulting in a high-performing, privacy-preserving system suitable for industrial deployment. 3) Scalablity with additional compute budget: In settings with high computational budgets, CHESS achieves $71.10\%$ accuracy on the BIRD test set, within $2\%$ of the leading proprietary method, while requiring approximately $83\%$ fewer LLM calls.

==> execution_trace.tex <==

In this section, we provide detailed execution traces of our pipeline, showcasing the output of each module. For example, as shown in figure \ref{fig:flowchart_926}, the effectiveness of our keyword extraction module is highlighted. It successfully identifies crucial values, such as ``Lewis Hamilton," which are necessary for constructing SQL queries. These identified keywords aid in retrieving database values and relevant column descriptions for input to the LLM.

In the entity retrieval sub-module, each keyword extracted is first broken down into individual words by splitting on spaces. This process makes our search order invariant, as entities mentioned in the question do not necessarily follow the same format as those in the database. Subsequently, for each keyword, the most similar database values are extracted. Likewise, all detected keywords are used to filter column descriptions, which are then provided for subsequent steps. This strategic provision of relevant information facilitates further processes, such as schema selection and query generation, thereby enhancing the accuracy of schema detection and SQL query formulation.

\begin{figure*}[h]
        \centering
        \includegraphics[width=\textwidth]{figures/trace_926.pdf}
        \caption{Execution flowchart for instance formula\_1\_926}
        \label{fig:flowchart_926}
\end{figure*}

In \ref{fig:flowchart_32}, we present a more challenging scenario where the question and evidence do not directly reference the relevant column names. The query mentions ``schools with the ownership code 66," yet no column explicitly includes ``ownership" in its name. In this case, the relevant column is "SOC" column from the schools table. The connection between this column and the question can only be discerned through the semantic similarity between the column descriptions and the question. Here, our context retrieval node plays a crucial role, as it effectively retrieves the relevant information from the database catalog, which is essential for answering this question.

\begin{figure*}[h]
        \centering
        \includegraphics[width=\textwidth]{figures/trace_32.pdf}
        \caption{Execution flowchart for instance California Schools\_32}
        \label{fig:flowchart_32}
\end{figure*}

==> introduction.tex <==
%%% General text-to-SQL background challenges

Translating natural language questions into database queries, commonly known as text-to-SQL, is a longstanding research challenge. The growing complexity of databases in recent years has exacerbated this problem, due to the increasing sizes of schemas (sets of columns and tables), values (content), and catalogs (metadata describing schemas and values) stored within them. Even some of the largest proprietary models, such as GPT-4, lag significantly behind human performance on text-to-SQL benchmarks, with a notable accuracy gap of 40\% \citep{li2024can}. Beyond the complexity of writing SQL queries, this substantial gap is primarily caused by the need to effectively retrieve and integrate multiple sources of information, including database values, catalogs, and schema, each in different formats, which complicates the process. Considering all these complexities, the lack of a robust verification method during the inference stage of text-to-SQL systems can undermine the reliability of their output query.

In Figure \ref{fig:intro_examples}, we illustrate some of the challenges facing modern text-to-SQL systems. For instance, users' questions might not directly match the stored values in the database, making it crucial to accurately identify the value format for effective SQL query formulation. Additionally, real-world database schemas often contain ambiguous column names, table names, and messy data, further complicating the SQL translation process and necessitating a robust retrieval system to identify relevant information. Moreover,  some questions may be inherently ambiguous, leading large language models (LLMs) to make subtle mistakes when generating SQL queries. For example, for the question illustrated on the right side of the Figure \ref{fig:intro_examples}, one might use 'ORDER BY' and 'LIMIT 1' to find the highest average score, while another approach could involve a subquery with the 'MAX()' function, potentially resulting in different outputs. 

Earlier work in the field \citep{pourreza2024din, wang2023mac, qi2022rasat, rajkumar2022evaluating, li2024pet} has generally limited the context for SQL generation to table structures, column definitions, and sample rows. However, in production-level databases, the database catalog and database values constitute a rich source of information that is crucial for generating accurate SQL queries. %These important sources are often overlooked in the field. 


%%% CHESS multi-agent framework for text-to-SQL

We introduce ``CHESS: contextual harnessing for efficient SQL synthesis", a multi-agent text-to-SQL system that designed to handle real-world and complex databases. The CHESS framework consists of four agents, each specialized for a specific task and equipped with effective tools: Information Retriever (IR), Schema Selector (SS), Candidate Generator (CG), and Unit Tester (UT). 

%%% Introducing agents with their tools

For the Information Retriever (IR) agent aims to retrieve the relevant entities (values in the database) and context (schema descriptions provided in database catalog). To achieve this, we present scalable and efficient methods using locality-sensitive hashing to retrieve database values from millions of rows, leveraging keyword detection, and vector databases to extract contextual information from database catalogs. Our approach utilizes both semantic and syntactic similarities between the database content and the user's query to enhance SQL prediction accuracy. 

As some previous work (needle-in-a-haystack) and our ablation studies (?) confirms, overloading the LLM context with redundant information can degrade its performance on downstream task. 
To address this, the Schema Selector (SS) agent is specifically designed to prune very large database schemas, allowing the candidate generator agent (CG) to perform a more effective reasoning when synthesizing SQL queries. This SS agent is equipped with three tools, \emph{filter_column}, \emph{select_tables}, and \emph{select_columns}, which allow it to maintain a scalable performance even with complex, real-world schemas with more than 4000 columns.

The Candidate Generator (CG) agent is responsible for writing SQL queries for the question asked from the database. After writing the queries, it executes them on the database, checks the results, and revises the queries if necessary.

Finally, the Unit Tester (UT) agent verifies the quality of the final query from different aspects. It generates multiple natural language unit tests and evaluates the generated candidate queries against them. UT then assigns a score to each of the candidates based on the number of unit tests that they pass and selects the one with the highest score. This verification approach ensures a more robust and reliable generation of the final query.

This team of agents works together to address the key challenges of text-to-SQL systems. The Information Retriever (IR) handles complex data retrieval, while the Schema Selector (SS) prunes large and ambiguous schemas to streamline query generation. The Candidate Generator (CG) refines SQL queries through execution, and the Unit Tester (UT) acts as a verifier, addressing noise and ambiguity by validating queries with natural language tests. Together, these agents tackle the performance gap and improve accuracy in real-world, complex databases.

%%% Different constraints in deployemnt ...

Despite significant advancements in text-to-SQL research, deploying such systems in industrial settings remains challenging. Key obstacles include 1) difficulties in scaling for highly complex industrial database schemas, 2) limited computational resources, and 3) concerns over data privacy. To address these challenges, we designed CHESS as a configurable framework that can adapt to various constraints.

For complex schemas (1), the Schema Selector (SS) agent efficiently narrows down large schemas into a manageable sub-schema, ensuring sufficient information to answer the query. Regarding computational limits (2), while previous work (such as CHASE and MTC-SQL) relies on frequent, costly LLM calls, CHESS achieves comparable performance using less powerful models, making it more suitable for resource-constrained environments. Finally, to address privacy concerns (3), we tested CHESS with fully open-source models that can be deployed on-premise, eliminating the need to send private data to third-party providers. Remarkably, CHESS outperformed other open-source baselines in these tests. In conclusion, CHESS offers a flexible solution capable of addressing the key challenges that hinder the deployment of text-to-SQL systems in industrial environments.

%%% Talking about ablation studies 


%%% General experiments on BIRD



%%% Contributions
- Novel multi-agent framework that breaks down the task into separate concerns ...
    - steerability, interpretability, ...


- Efficient hierarchical design for retrieving the information 
- Scalable schema selection protocol

- 
- SOTA on end-to-end open-source LLMs
- First to design, (NL) Unit test generation for text-to-SQL


==> methodology.tex <==
The text-to-SQL task is a challenging learning problem, requiring models to translate a natural language question and database schema into a valid SQL query. The input consists of the text of the question, the database schema defining table structures and column types, and the database instance containing the table content. Additionally, the input may include a database catalog containing metadata, which allows for free-form textual attribute values. Key challenges in this task include handling noisy database content, capturing implicit semantic correspondences between input elements, and mapping a, potentially ambiguous, natural language question to SQL's compositional and formal query structure.

``CHESS: Contextual Harnessing for Efficient SQL Synthesis" is a multi-agent text-to-SQL system designed for complex, real-world databases. 
It introduces a scalable and effective framework consisting four main agents: Information Retriever (IR), Schema Selector (SS), Candidate Generator (CG), and Unit Tester (UT). Each agent is equipped with specialized tools to achieve its objectives. For instance, the IR agent has access to \emph{retrieve\_entity} tool which, powered by a preprocessed locality-sensitive hashing index, allows it to retrieve relevant database values efficiently. In the following, we provide a detailed explanation of each agent's functionality and tools. See Figure ?? for an illustration of the framework.

Finally, real-world deployment of text-to-SQL systems must consider various constraints, such as the reasoning capabilities and sampling budgets of large language models (LLMs), as well as data privacy concerns. CHESS is designed as a configurable framework that can adapt to different deployment scenarios while maintaining high performance. In section ??, we discuss various deployment settings and how CHESS can be customized to meet performance requirements while adhering to these constraints.



\subsection{Agents}

Detailed implementation and prompt examples are provided in Appendix ??.

\paragraph{Information Retriever (IR)} The information retriever agent equipped with the tools, \emph{extract_keywords}, \emph{entity_retriever}, and \emph{context_retriever}, gathers relevant information related to the input, including entities mentioned in the question and the contextual information provided in the database catalog. The tools are described as follows:

\vspace{-0.7em}
\paragraph{\emph{extract\_keywords}).}
To search for the similar values in the database and schema description, the agent needs to extract the main keywords from the natural language question. This tool uses a few-shot LLM call to extract the primary keywords and key phrases from the input.

\vspace{-0.7em}
\paragraph{\emph{retrieve_entity}.}
From the list of keywords extracted from the question, some may correspond to entities present in the database. This tool allows the agent to search for similar values in the database and return the most relevant matches, along with their corresponding columns, for each keyword.  
To assess syntactic similarity between the keywords and the database values, we employ the edit distance similarity metric. Additionally, to enhance retrieval efficiency, we propose a hierarchical retrieval strategy based on \hyperlink{subsubsec:lsh_indexing}{Locality Sensitive Hashing (LSH)} and semantic (embedding) similarity measures, which we explain in detail in Appendix \ref{sec:implementation_details}. This approach enables the agent to retrieve values that exhibit both syntactic and semantic similarity to the keywords effectively.

\vspace{-0.7em}
\paragraph{\emph{retrieve_context}.}
In addition to retrieving values, the IR agent can access the database catalog, which often includes schema metadata, such as column descriptions, extended column names (to resolve abbreviations), and value descriptions. As shown in Figure~\ref{fig:intro_examples}, this information can be useful, and not providing it to the model can lead to suboptimal performance. The IR agent uses this tool to retrieve the most relevant descriptions from the database catalog by querying a \hyperlink{subsubsec:vector_database}{vector database of descriptions}, constructed during the preprocessing. Retrieval is based on semantic (embedding) similarity, ensuring that the most relevant context is provided to the model.


\paragraph{Schema Selector (SS)} The goal of the Schema Selector (SS) agent is to reduce the schema size by selecting only the necessary tables and columns required for generating the SQL query. To achieve this, the SS agent is equipped with three tools, \emph{filter_column}, \emph{select_tables}, and \emph{select_columns}. 

\paragraph{\emph{filter_column}} Databases often contain hundreds of columns, many of which may be semantically irrelevant to the user's query. Inspired by this observation, we design this tool which takes a column name and the question as input and determines whether the column is relevant. While this task could be perform using embedding-based similarity methods, we opt for a relatively inexpensive LLM to ensure high accuracy. %% should we keep this sentence?

Although this tool is effective at filtering out irrelevant columns, identifying relevant schema elements accurately often requires processing multiple schema items together. The following tools complement this process by handling such scenarios.  

\paragraph{\emph{select_tables}} This tool takes a sub-schema of the database and the question as input, and through LLM prompting, returns the tables that are necessary for answering the query.

\paragraph{\emph{select_columns}} To further narrow down the relevant schema items, the \emph{select_columns} tool can be used. By inputting a sub-schema and the question, the agent retrieves only the necessary columns.

The SS agent can use any of these tools individually or in combination, depending on its configuration. However, its actions introduce a trade-off between precision and recall in selecting useful schema items. The effectiveness of these tools depends on the specific setup of the LLMs and the complexity of the database schema. A detailed discussion of this trade-off is presented in section ??.


\paragraph{Candidate Generator (CG)} The Candidate Generator (CG) is responsible for synthesizing SQL query that answers the question asked from the database. To accomplish this, the CG agent first calls the \emph{generate_candidate_query} tool to generate candidate queries. It then executes these candidates on the database, checks the result, and identifies any faulty queries (those containing syntactic errors or empty result). For each faulty candidate, the agent repeatedly attempts to \emph{revise} the query, until the issue is resolved or a maximum number of allowed revisions is reached.   

\paragraph{\emph{generate_candidate_query}} This tool generates a single candidate query that answers the question. It takes the question, the schema, and the context (entities and descriptions) and prompts an LLM to follow a multi-step reasoning guideline to write a candidate SQL query. 

\paragraph{\emph{revise}} Sometimes, the generated candidate queries may contain syntax errors or produce empty result. In such cases, the agent identifies the issue by executing the queries on the database and then uses this tool to fix them. This tool takes the question, schema, context, the faulty query and a description of the issue as input. It then prompts an LLM with this information, asking it revise the query. Note that the issue description (or execution log) is critical in guiding the model, as it provides a direct signal of the query's failure point.


\paragraph{Unit Tester (UT)} The Unit Tester (UT) agent is responsible for selecting the most accurate SQL query from the pool of candidates generated by the CG agent. UT identifies the best candidate by 1) generating multiple unit tests that highlight differences between the candidate queries and 2) evaluating the candidates against these unit tests. It then assigns a score to each query based on the number of unit tests it passes, selecting the top-scoring candidate as the final SQL query for the given question.

\paragraph{\emph{generate_unit_test}} This tool prompts an LLM to generate $k$ unit tests, where $k$ is an input parameter, designed such that only the correct SQL query can pass them. The prompt is carefully constructed to produce high-quality unit tests that highlight the semantic differences between the candidate queries. Detailed explanations of the implementation and prompt are provided in Appendix ??.

\paragraph{\emph{evaluate}} After generating the unit tests, the UT agent evaluates the candidate queries against them. This tool takes multiple candidate queries and a single unit test as input, prompting an LLM to reason through each candidate and determine whether it passes the unit test. While this tool could be implemented to evaluate a single candidate against multiple unit tests simultaneously, ablation studies (??) have shown that the current approach, evaluating multiple candidates against one unit test at a time, yields better results.

\subsection{Preprocessing}
\label{subsec:preprocessing}
\vspace{-0.3em}

To accelerate the IR agent's tools, \emph{retrieve\_entity} and \emph{retrieve\_context}, and improve their efficiency, we preprocess database values and catalogs before executing the pipeline. For database values, we perform a syntactic search by creating a Locality-Sensitive Hashing (LSH) index, as explained in \emph{retrieve\_entity}. For database catalogs, which contain longer texts that require semantic understanding, we use a \hyperlink{subsubsec:vector_database}{vector database} retrieval method to measure semantic similarity.

\vspace{-0.7em}
\hypertarget{subsubsec:lsh_indexing}{\paragraph{Locality Sensitive Hashing Indexing of Values.}}

To optimize the entity retrieval process, we employ a method capable of efficiently searching through large databases, which may contain millions of rows, to retrieve the most similar values. This process doesn't require perfect accuracy but should return a reasonably small set of similar values, such as around a hundred elements.
Locality Sensitive Hashing (LSH) is an effective technique for approximate nearest-neighbor searches, allowing us to retrieve database values most similar to a given keyword. During preprocessing, we index unique database values using LSH. Then, in the \emph{retrieve\_entity} tool, we query this index to quickly find the top similar values for a keyword.

\vspace{-0.7em}
\hypertarget{subsubsec:vector_database}{\paragraph{Vector Database for Descriptions.}}

As explained in \hyperlink{subsubsec:context_retrieval}{context retrieval}, extracting the most semantically relevant pieces of information from database catalogs is crucial for generating accurate SQL queries. These catalogs can be extensive, with hundreds of pages explaining the entities and their relationships within the database, necessitating an efficient retrieval method.
To enable a high-efficiency semantic similarity searches, we preprocess the database catalogs into a vector database. During the context retrieval step, we query this vector database to find the most relevant information for the question at hand.


For a more detailed description of our framework and the preprocessing phase, please refer to Appendix \ref{sec:implementation_details}.

\subsection{Handling real-world constraints} Deploying a text-to-SQL system in real-world environments requires navigating a variety of constraints, such as the availability of computational resources, the reasoning budget for large language models (LLMs), and data privacy concerns. To accommodate these different constraints, CHESS is designed as a configurable framework, capable of adapting to various deployment scenarios.

In setups where higher computational budgets and more powerful LLMs are available, CHESS can be configured to maximize accuracy by leveraging these resources. Specifically, the Candidate Generator (CG) and Unit Tester (UT) agents can be programmed to generate multiple candidate queries and unit tests, leading to more accurate final SQL queries \cite{monkey}. This increased sampling allows the system to refine its query generation process, resulting in better performance.

Interestingly, similar to the findings in \cite{distillery}, we observed that when schema sizes are relatively small and the available LLMs are highly capable, the inclusion of the Schema Selector (SS) agent may introduce a precision-recall trade-off that can negatively impact accuracy. In these cases, omitting the SS agent can lead to better results. However, as we will demonstrate in Section ??, for larger schemas, even powerful LLMs struggle to maintain performance. In such cases, the collaboration of all four agents is essential for achieving higher accuracy, as the SS agent becomes crucial for managing the complexity of the schema.

In contrast, when computational resources are limited or when only weaker LLMs—such as small open-source models—are available to ensure data privacy, CHESS can be reconfigured for efficiency. In these scenarios, we streamline the system by excluding the UT agent and limiting the CG agent to generate only one candidate query. This approach minimizes computational overhead while still synthesizing a reliable SQL query, making CHESS suitable for resource-constrained environments.
